Jamming Attacks and Anti-Jamming Strategies in Wireless Networks: A Comprehensive Survey

Wireless networks are a key component of the telecommunications infrastructure in our society, and wireless services become increasingly important as the applications of wireless devices have penetrated every aspect of our lives. Although wireless technologies have significantly advanced in the past decades, most wireless networks are still vulnerable to radio jamming attacks due to the openness nature of wireless channels, and the progress in the design of jamming-resistant wireless networking systems remains limited. This stagnation can be attributed to the lack of practical physical-layer wireless technologies that can efficiently decode data packets in the presence of jamming attacks. This article surveys existing jamming attacks and anti-jamming strategies in wireless local area networks (WLANs), cellular networks, cognitive radio networks (CRNs), ZigBee networks, Bluetooth networks, vehicular networks, LoRa networks, RFID networks, and GPS system, with the objective of offering a comprehensive knowledge landscape of existing jamming/anti-jamming strategies and stimulating more research efforts to secure wireless networks against jamming attacks. Different from prior survey papers, this article conducts a comprehensive, in-depth review on jamming and anti-jamming strategies, casting insights on the design of jamming-resilient wireless networking systems. An outlook on promising antijamming techniques is offered at the end of this article to delineate important research directions.

==> other_networks.tex <==
In this section, we survey jamming and anti-jamming attacks in GPS, Radar and RFID wireless communication systems. 
We first provide an introduction on these systems, and then review the jamming/anti-jamming techniques uniquely designed for these systems. 

\begin{figure}
	\centering
	\includegraphics[width=2.9in]{figures/gps_attack.pdf}
	\caption{Security attack on GPS networks.}
	\label{fig:gps_attack}
\end{figure}



\subsection{GPS Communication Systems}

\subsubsection{A Primer}

\begin{figure}[t]
	\centering
	\includegraphics[width=3.5in]{figures/gps_frame.pdf}
	\caption{GPS navigation message frame structure.}
	\label{fig:gps_frame}
\end{figure}


\begin{figure}[t]
	\centering
	\includegraphics[width=2.5in]{figures/gps_receiver.pdf}
	\caption{GPS receiver structure \cite{karaim2019ultra}}
	\label{fig:gps_frame}
\end{figure}


In this section, we will overview the concept of GPS service as well as its physical layer signaling.
Simply put, the GPS satellites orbiting around the earth continuously broadcast their location and time information.
%
Once a user acquires a satellite's time and location information, it can estimate its distance, known as pseudo range, from the satellite by calculating the time the signal lasted to arrive and simply multiplying it by the speed of light.
%
The user's geographical location can be later determined mathematically using the estimated pseudo ranges and the locations of multiple satellites.

The satellites provide the required information for the users via broadcasting navigation messages.
Fig. \ref{fig:gps_frame} shows the structure of a GPS navigation message.
A navigation message consists of $5$ equally-sized subframes of $10$ data words.
%
Data words consist of $24$ raw data bits followed by $6$ parity bits.
%
The first data word in each subframe is telemetry (TLM) word which is a binary preamble and used for start of subframe detection as well as administrative status information.
%
following the TLM word is Handover (HOW) word and carries GPS system time information which is used to identify the subframe. 
Subframe $1$ carries the information required for clock offset estimation. 
%
Subframes $2$ and $3$ consist of satellite ephemeris data that can be used by the users to accurately estimate the satellite's location at a particular time. 
%
Subframes $4$ and $5$ carry almanac data that provides information on all satellites and their orbits on the constellation.


The navigation message is sent with $50$~bps data rate.
All GPS satellites operate in $1575.42$~MHz (L1 channel) and $1227.60$~MHz (L2 channel) and use on of the following signaling protocols;\\
\textbf{Course Acquisition (C/A) code:} C/A signal uses direct sequence spread spectrum (DSSS) with a 1023-chip pseudo random spreading sequence which is replicated $20$ times in order to achieve higher spreading gain. 
%
The main lobe C/A signal bandwidth is $2$~MHz and the spreading gain is $10 \times \log_{10}(20 \times 1023) \approx 43$~dB.
%
The C/A signal is transmitted over L1 frequency channel and mainly used to serve civilian users.

\noindent
\textbf{P code:}
P code signal also uses spreading spectrum. 
%
The length of spreading code is $10230$~chips per bit for the P code signal.
%
P signals is more spreaded over the frequency and can achieve higher spreading gain ($\approx 53$~dB) compared to C/A signal.
%
The signal bandwidth is $20$~MHz for P code signal.
%
P signal can be transmitted over both the L1 and L2 channels, and is designed by the US Department of Defense for authorized users.

%
\subsubsection{Jamming Attacks}

GPS signal can be easily drowned by conventional jamming signals due to its low power.
In \cite{glomsvoll2014jamming}, the GPS receiver performance is analyzed under jamming attacks. 
A wide-band commercial of the shelf jammer at the L1 carrier frequency has been used to jam the GPS signal on board.
%
Signal spoofing is another critical security threat to the GPS systems.
GPS spoofing can be used to falsify the navigation estimation and timing synchronization. 
In \cite{warner2002simple,humphreys2008assessing,motella2010performance}, the authors analyze the performance of civilian GPS receivers under practical GPS spoofing. 
%
In addition to global location, GPS system provides time information for GPS receivers.
This time information provides time source in the range from microsecond to seconds for interoperability of many applications, where the system components are dispersed in different time-zone areas \cite{zeng2012gps}.
%
In \cite{kuhn2004asymmetric}, an attacker is designed to falsify the timing of military GPS signals by spoofing a delayed version of the signal.
 




\subsubsection{Anti-Jamming Attacks}

\noindent
\textbf{Jamming Signal Filtering:}
In \cite{zhang2001anti}, Zhang et al. proposed to design a mask in both time and frequency domains using the time and frequency distributions of the jamming signal to suppress its energy while passing the GPS signal.
%
In \cite{chien2013design}, an adaptive notch filter is designed to detect, estimate, and block single-tone continuous jamming signals.
The notch filter is simply designed in time domain and composed of a second-order IIR filter.
%
In \cite{rezaei2016new}, to enhance the jamming mitigation capability of notch filter, Rezaei et al. propose to use the short-time Fourier transform (STFT) to increase the time and frequency domain resolution.


\noindent
\textbf{Antenna Array Design:}
Antenna array processing is a well-known technique proposed for anti-jamming GPS receivers to suppress the jamming signal and enhance the desired signal \cite{li2014robust}.
In \cite{rezazadeh2019compact}, Rezazadeh et al. design an adaptive antenna system based on pattern and polarization diversity to nullify jamming signal in airborne GPS applications.
\cite{zhang2012anti} addresses the challenges associated with the antenna array design for GPS receiver.
Particularly, Zhang et al. propose an array-based adaptive anti-jamming algorithm to suppresses jamming signal with negligible phase distortion.
%
\cite{sun2005self} harnesses the inherent self-coherence feature of the GPS signals as it repeats $20$ times within each symbol to mitigate the jamming signal.
It uses the spectral self-coherence beamforming technique proposed in \cite{agee1990spectral} to design a weight vector that can remove the jamming signal and improve the desired signal detection.
%
A Similar idea has been proposed in \cite{lu2013global}, where the received signal is projected onto the orthogonal space of jamming signal and the CLEAN method proposed in \cite{schwarz1978mathematical} is used to iteratively design the beamforming vector to estimate direction of arrivals of multiple GPS signals.

% \subsection{Radar Sensing Systems}

% \subsubsection{A Primer}

% \subsubsection{Jamming Attacks}
% \cite{o2019overview} overviews the vulnerability of FM, DAB and DVB-T based passive radar systems under noise and single tone jamming attacks. 
% %
% In \cite{chen2016analyzing}, the impact of cybersecurity attacks on detection performance of a distributed MIMO radar has been investigated. 
% A distributed MIMO radar system consists of multiple transmitters, receivers, and a fusion center where the final target detection decision is made. 
% A distributed MIMO radar offers improved performance compared with a conventional radar system due to the increased system diversity and degrees of freedom.


% \subsubsection{Anti-Jamming Techniques}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \caption{Jamming attacks and anti-jamming techniques in GPS communications}
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \cellcolor[HTML]{EFEFEF}                                                                     & \multicolumn{1}{c|}{\textbf{Ref.}}                                     & \multicolumn{1}{c|}{\textbf{Description}}                                                                     \\ \hline
%                                                                                              & \cite{glomsvoll2014jamming}                                           & GPS receiver performance analysis under wide-band commercial jamming attacks.                                 \\ \cline{2-3} 
%                                                                                              & \cite{warner2002simple,humphreys2008assessing,motella2010performance} & GPS signal spoofing.                                                                                          \\ \cline{2-3} 
%                                                                                              & \cite{zeng2012gps}                                                    & GPS time information attack.                                                                                  \\ \cline{2-3} 
% \multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Jamming \\ attacks\end{tabular}}}        & \cite{kuhn2004asymmetric}                                             & Falsify the timing of military GPS signals using spoofing.                                                    \\ \hline
%                                                                                              & \cite{zhang2001anti}                                                  & Mask design in time and frequency domain using the time and frequency distributions of the jamming signal.    \\ \cline{2-3} 
%                                                                                              & \cite{chien2013design}                                                & Adaptive notch filter design to detect, estimate, and block single-tone continuous jamming signals.           \\ \cline{2-3} 
%                                                                                              & \cite{rezaei2016new}                                                  & Short-time Fourier transform (STFT) use to enhance resolution in notch filter design.                         \\ \cline{2-3} 
%                                                                                              & \cite{li2014robust}                                                   & Antenna array design.                                                                                         \\ \cline{2-3} 
%                                                                                              & \cite{rezazadeh2019compact}                                           & Adaptive antenna system design based on pattern and polarization diversity.                                   \\ \cline{2-3} 
%                                                                                              & \cite{zhang2012anti}                                                  & Adaptive array-based algorithm with negligible phase distortion.                                              \\ \cline{2-3} 
%                                                                                              & \cite{sun2005self}                                                    & Spectral self-coherence beamforming technique considering inherent self-coherence feature of the GPS signals. \\ \cline{2-3} 
% \multirow{-8}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Anti-jamming\\ techniques\end{tabular}}} & \cite{lu2013global}                                                   & Received signal projection onto the orthogonal space of jamming signal.                                       \\ \hline
% \end{tabular}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\caption{Jamming attacks and anti-jamming techniques in GPS and RFID communications}
\begin{tabular}{|ll|l|l|}
\hline
\cellcolor[HTML]{EFEFEF}                                                                                    & \cellcolor[HTML]{EFEFEF}       & \multicolumn{1}{c|}{\textbf{Ref.}}                                     & \multicolumn{1}{c|}{\textbf{Description}}                                                                                                                        \\ \hline
\multicolumn{1}{|l|}{}                                                                                      &                                & \cite{glomsvoll2014jamming}                                           & Analyzed GPS receiver performance under wide-band commercial jamming attacks.                                                                                    \\ \cline{3-4} 
\multicolumn{1}{|l|}{}                                                                                      &                                & \cite{warner2002simple,humphreys2008assessing,motella2010performance} & Investigated the GPS signal spoofing.                                                                                                                            \\ \cline{3-4} 
\multicolumn{1}{|l|}{}                                                                                      &                                & \cite{zeng2012gps}                                                    & Studied the GPS time information attack.                                                                                                                         \\ \cline{3-4} 
\multicolumn{1}{|l|}{\multirow{-4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Jamming \\ attacks\end{tabular}}}} & \multirow{-4}{*}{\textbf{GPS}} & \cite{kuhn2004asymmetric}                                             & Used spoofing attack to falsify the timing of the military GPS signals.                                                                                          \\ \cline{2-4} 
\multicolumn{1}{|l|}{\textbf{}}                                                                             &                                & \cite{fu2010research}                                                 & Investigated the impact of constant jamming attacks on UHF RFID communications.                                                                                  \\ \cline{3-4} 
\multicolumn{1}{|l|}{}                                                                                      & \textbf{RFID}                  & \cite{mitrokotsa2010classifying}                                      & Introduced zapping attack on RFID communications.                                                                                                                \\ \cline{3-4} 
\multicolumn{1}{|l|}{}                                                                                      &                                & \cite{oren2012rfid,oren2009attacks}                                   & Investigated the impact of constant jamming attack and zapping attack on RFID-based e-voting.                                                                    \\ \hline
\multicolumn{1}{|l|}{\textbf{}}                                                                             & \textbf{}                      & \cite{zhang2001anti}                                                  & Designed a time-frequency mask using the time and frequency distributions of the jamming signal.                                                                 \\ \cline{3-4} 
\multicolumn{1}{|l|}{\textbf{}}                                                                             &                                & \cite{chien2013design}                                                & Used adaptive notch filter design to detect, estimate, and block single-tone continuous jamming signals.                                                         \\ \cline{3-4} 
\multicolumn{1}{|l|}{\textbf{}}                                                                             &                                & \cite{rezaei2016new}                                                  & Used short-time Fourier transform (STFT) to enhance resolution in notch filter design.                                                                           \\ \cline{3-4} 
\multicolumn{1}{|l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Anti-jamming\\ techniques\end{tabular}}}            & \textbf{GPS}                   & \cite{li2014robust}                                                   & Designed an adaptive antenna array.                                                                                                                              \\ \cline{3-4} 
\multicolumn{1}{|l|}{\textbf{}}                                                                             &                                & \cite{rezazadeh2019compact}                                           & Designed an adaptive antenna system based on pattern and polarization diversity.                                                                                 \\ \cline{3-4} 
\multicolumn{1}{|l|}{\textbf{}}                                                                             &                                & \cite{zhang2012anti}                                                  & Proposed an adaptive array-based algorithm with negligible phase distortion.                                                                                     \\ \cline{3-4} 
\multicolumn{1}{|l|}{\textbf{}}                                                                             &                                & \cite{sun2005self}                                                    & \begin{tabular}[c]{@{}l@{}}Proposed spectral self-coherence beamforming technique considering inherent self-coherence\\ feature of the GPS signals.\end{tabular} \\ \cline{3-4} 
\multicolumn{1}{|l|}{\textbf{}}                                                                             &                                & \cite{lu2013global}                                                   & Used received signal projection onto the orthogonal space of jamming signal.                                                                                     \\ \cline{2-4} 
\multicolumn{1}{|l|}{}                                                                                      & \textbf{RFID}                  & \cite{avanco2015effective}                                            & Proposed a low-power jamming attack detection mechanism for RFID communications.                                                                                 \\ \hline
\end{tabular}
\end{table*}



\subsection{RFID Communication Systems}

\subsubsection{A Primer}
Radio-frequency identification (RFID) is an enabling technology that allows an interrogator (reader) to read the information stored in simple-designed tags attached to different objects such as humans, animals, cars, clothes, books, grocery products, jewelry, and etc. from short distances using electromagnetic waves.
%
RFID tags can be in general passive or active.
Passive tags refers to the tags that do not have battery and use energy harvesting for their transmissions.
Active tags on the other hand use battery to drive their RF circuits.

An RFID reader manages an UHF RFID tag population using following three main phases:

\noindent
\textbf{Select:} The reader selects a tag population by sending \textit{select} commands by which a group of tags are informed for further inquiry process.

\noindent
\textbf{Inventory:} In this phase, the reader identifies the selected tags. 
%
The inventory rounds are initialized by the reader issuing \textit{Query} commands. 
%
The reader and RFID tags communicate using slotted ALOHA medium access mechanism.
%
Upon a new-selected tag receives a Query command, it will set its counter to a pseudo-random number.
%
Every time it receives the Query command it decreases its counter by $1$.
%
When the tag's counter reaches to zero, it responds the reader by a 16-bit pseudo-random sequence (RN16).
%
The reader acknowledges the RN16 signal reception by regenerating the same RN16 and sending it back to the tag.
%
When the tag receives the replied RN16 signal, compares it with the original transmitted one. 
%
If they are matched, the tag will broadcast its EPC and the reader will identify the tag.

\noindent
\textbf{Access:} When the inventory phase is completed, the reader can access the tag.
%
In this phase, the reader may write/read to/from the tag's memory, kill, or lock the tag.
%
From PHY-layer perspective, an UHF RFID readers use pulse interval encoding (PIE) encoding and DSB-ASK/SSB-ASK/PR-ASK modulation for its data transmission, while an UHF RFID tag uses FM0 or Miller data encoding and backscattering for carrier modulation.
%
Moreover, the required energy for the tag's backscattering is delivered via the reader's continuous wave (CW) transmissions.




\subsubsection{Jamming Attacks}
\begin{figure}
	\centering
	\includegraphics[width=2.8in]{figures/rfid_attack.pdf}
	\caption{Jamming attack on a RFID network.}
	\label{fig:rfid_attack}
\end{figure}

In \cite{fu2010research}, Fu et al. investigated the impact of constant jamming attack on UHF RFID communications and evaluated the system performance through a simulation model.
The results in \cite{fu2010research} showed that when the received RFID reader signal power is $0$~dBm, the received jamming signal power of $-15$~dBm will be sufficient to break down the RFID communications.
Zapping attack is one of the well-known security attacks to RFID tags, in which the attacker targets the RF front-end circuits in RFID tags to destroy.
In this class of attacks, the adversary attacker produces a strong electromagnetic induction through the tag's circuit by generating a high-power signal in the proximity of the tag's antenna.
The large amount of energy the tag receives causes permanent damage to its RF circuits \cite{mitrokotsa2010classifying}.

RFID tags are recently used for electronic voting systems in many countries across the world where the votes are written through the RFID tags electronically instead of conventional ballot voting papers.
Electronic voting systems are originally designed to improve the accuracy and pace of vote counting process.
Considering the importance of the service made the RFID security to receive a large amount of attention from both academia and industrial.
In \cite{oren2012rfid,oren2009attacks}, Oren et al. studied two main security threats, jamming and zapping attacks, on RFID communications.
The authors conducted two jamming attacks, constant jamming attack and a modulated clock signal corresponding to RFID tag's sampling rate, and evaluated their performances in terms of the maximum range jammer is capable to completely block the RFID communications.
The author also investigated the impact of the jammer's antenna type on its performance. 
It was shown that the helical antennas can support higher range compared to hustler and $39$~cm loop antennas to achieve the same performance degradation.

In \cite{rieback2006evolution}, Rieback et al. divided the security threats against RFID communications into following items;

\noindent
\textbf{Spoofing Attack:} In this class of attack, the attacker accesses to the tag's memory blocks and changes the tag's information such that it is still meaningful to the reader but carries false data.   

\noindent
\textbf{Denial of Service Attack:} It refers to the scenario in which the reader will no longer be able to read data from its corresponding tags.
Per \cite{rieback2006evolution}, DoS attack in RFID communications can be performed either by physically isolating the tags (e.g., wrapping the tags in foils) so the reader can not deliver the required energy for tag's backscattering, or by injecting a large amount of data into medium that the reader cannot manage.

\noindent
\textbf{Replay attack:} In \cite{danev2012physical}, Danev et al. introduced replay attack where the attacker receives the tag's signal, stores it, and re-uses it in different time slots.

\noindent
\textbf{Passive Attack:} Passive attack was argued as one of the main security vulnerabilities in RFID communications, as the tags EPC information can be read by any commercial off-the-shelf or custom-designed interrogators.
Moreover, Cho et al. in \cite{cho2015consideration} proposed brute-force attack in which the attacker uses brute-forcing algorithms to pass the tag's authentication procedure, where it can write/read to/from the tag.
The recorded data from RFID tags can be further used for object tracing, or spoofing attack.

% \textbf{Tag cloning: \cite{}} \\
% \textbf{Man-in-the-middle attack:\cite{} }
% \\





\subsubsection{Anti-Jamming Techniques}
Despite of many works done in literature to address the security threats in RFID communications, there are very limited research papers associated with PHY-layer techniques for jamming mitigation.
Most of the existing works focus on authentication level security issues. 

For example, in \cite{wang2020hu}, Wang et al. proposed an authentication level solution in order to cope with RFID replay attack.
In \cite{avanco2015effective}, Avanco et al. proposed a low-power jamming attack detection mechanism in RFID networks.
Their proposed scheme takes the receive signal powers in adjacent channels as well as the received tag's preamble and the tag's uplink transmissions' responses into account in order to identify any malicious activities within the network.


% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \caption{Jamming attacks in other wireless systems.}
% \begin{tabular}{|l|p{1.5cm}|l|}
% \hline
%                                              & \multicolumn{1}{c|}{\textbf{Ref}}                                      & \multicolumn{1}{c|}{\textbf{Description}}                                                            \\ \hline
% \multirow{2}{*}{\textbf{VANETs}}             & \cite{azogu2013new,punal2012vanets,punal2014experimental}             & Conventional jamming attacks’ impact on IEEE 802.11p-based V2V communications.                       \\ \cline{2-3} 
%                                              & \cite{sumra2011behavior,sumra2014effects}                             & Data integrity attack.                                                                               \\ \hline
% \multirow{2}{*}{\textbf{UAVs}}               & \cite{hartmann2013vulnerability}                                      & UAVs' satellite communication jamming attack.                                                        \\ \cline{2-3} 
%                                              & \cite{rudinskas2009security}                                          & UAVs' control command jamming attack.                                                                \\ \hline
% \multirow{4}{*}{\textbf{GPS communications}} & \cite{glomsvoll2014jamming}                                           & GPS receiver performance analysis under wide-band commercial jamming attacks.                        \\ \cline{2-3} 
%                                              & \cite{warner2002simple,humphreys2008assessing,motella2010performance} & GPS signal spoofing.                                                                                 \\ \cline{2-3} 
%                                              & \cite{zeng2012gps}                                                    & GPS time information attack.                                                                         \\ \cline{2-3} 
%                                              & \cite{kuhn2004asymmetric}                                             & Falsify the timing of military GPS signals using spoofing.                                           \\ \hline
% \textbf{Radar communications}                & \cite{o2019overview}                                                  & Vulnerability studies of FM, DAB and DVB-T based passive radar systems under various jamming attack. \\ \hline
% \end{tabular}
% \end{table*}













==> overview.tex <==


\subsection{Jamming Vulnerability of Wireless Networks}
 

\subsection{Jamming Attack Strategies}
\subsubsection{Constant Jamming Attacks}
\subsubsection{Reactive Jamming Attacks}
\subsubsection{Proactive Jamming Attacks}
\subsubsection{Protocol-Aware Jamming Attacks}



%
\subsection{Anti-jamming Techniques}
\subsubsection{Power Control Techniques}
\subsubsection{Spatial Domain Techniques}
\subsubsection{Frequency Hopping Techniques}
\subsubsection{Coding Techniques}




==> tab_survey_crn.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\caption{A summary of jamming and anti-jamming attacks in cognitive radio networks.}
\centering
\begin{tabular}{|l|l|l|}
\hline
& \multicolumn{1}{c|}{\textbf{Ref.}} & \multicolumn{1}{c|}{\textbf{Description}}   \\ \hline
\textbf{}  & \cite{jo2013selfish}  & Used PUE attack to vacate the spectrum for its exclusive usage. \\ \cline{2-3} 
   & \cite{chen2011cooperative}& Used malicious PUE attack to cause DoS in centralized cooperative spectrum sensing CRNs.\\ \cline{2-3} 
\multirow{-2}{*}{{PUE attacks}} & \cite{chen2009modeling}   & Designed an advance malicious PUE attack by taking the PU's receive power into account. \\ \hline
\textbf{}  & \cite{fatemieh2011using}  & \begin{tabular}[c]{@{}l@{}}Introduced selfish false-report attack where the attacker sends fake channel busy reports \\ to exclusively access the channel.\end{tabular} \\ \cline{2-3} 
   & \cite{chen2016joint,zhang2014performance} & Proposed an attack to report a value opposite to its local sensing decision to degrade the FC performance.  \\ \cline{2-3} 
\multirow{-2}{*}{\textbf{}}& \cite{fatemieh2010secure} & Designed an attack to report the channel as unused when it is busy to cause interference to the primary network.\\ \cline{2-3} 
   & \cite{chen2008robust,wang2010phy,abdelhakim2011cooperative}   & Studied false-report attack in centralized cooperative spectrum sensing.\\ \cline{2-3} 
\multirow{-2}{*}{{\begin{tabular}[c]{@{}l@{}}False-report \\ attacks\end{tabular}}} & \cite{akyildiz2009crahns,li2009distributed,bazerque2009distributed,ding2012decentralized} & Studied false-report attack in decentralized cooperative spectrum sensing networks. \\ \cline{2-3} 
   & \cite{kailkhura2013distributed}   & Proposed spectrum sensing protocol-aware false report attack.   \\ \cline{2-3} 
   & \cite{penna2011detecting} & Proposed probabilistic false report attack. \\ \cline{2-3} 
   & \cite{rawat2010collaborative} & Studied the impact of attack population on false-report attack performance. \\ \hline
{\begin{tabular}[c]{@{}l@{}}Common control \\ channel attacks\end{tabular}} & \cite{bian2006mac}& Evaluated the impact of jamming attack on common control channel.   \\ \hline
\textbf{}  & \cite{li2009dogfight} & Proposed random channel hopping against PUE attack. \\ \cline{2-3} 
   & \cite{chang2017jamming}   & Introduce Tri-CH, an anti-jamming channel hopping algorithm.\\ \cline{2-3} 
{\begin{tabular}[c]{@{}l@{}}Anti-jamming \\ techniques\end{tabular}}& \cite{wu2011anti} & Used zero-sum game modeling and a channel hopping defense strategy. \\ \cline{2-3} 
   & \cite{lo2012multiagent}   & \begin{tabular}[c]{@{}l@{}}Proposed JRCC game modeling; Cooperation for control channel allocation and adaptive \\ rate learning for primary user\end{tabular}  \\ \cline{2-3} 
   & \cite{wang2011anti}   & Proposed a game theoretical approach to model the CRN under jamming attack. \\ \cline{2-3} 
   & \cite{asterjadhi2010jenna}& Propose JENNA;  Random channel hopping and network coding for control packets sharing.  \\ \hline
\end{tabular}
\label{tab:summary_crn}
\end{table*}
